Differentially Describing Groups of Graphs

How does neural connectivity in autistic children differ from neural connectivity in healthy children or autistic youths? What patterns in global trade networks are shared across classes of goods, and how do these patterns change over time? Answering questions like these requires us to differentially describe groups of graphs: Given a set of graphs and a partition of these graphs into groups, discover what graphs in one group have in common, how they systematically differ from graphs in other groups, and how multiple groups of graphs are related. We refer to this task as graph group analysis, which seeks to describe similarities and differences between graph groups by means of statistically significant subgraphs. To perform graph group analysis, we introduce Gragra, which uses maximum entropy modeling to identify a non-redundant set of subgraphs with statistically significant associations to one or more graph groups. Through an extensive set of experiments on a wide range of synthetic and real-world graph groups, we confirm that Gragra works well in practice.

==> text/discussion.tex <==
% !TeX spellcheck = en_US
% !TeX root = paper.tex
%\section{Discussion}
%\label{sec:discussion}
%
%In our experiments, 
%we have shown that \ourmethod differentially describes synthetic and real-world graph groups. 
%As a byproduct, we have introduced two novel datasets of node-aligned graphs, 
%which might be of independent interest as a resource to the graph mining community.
%However, our work also has several limitations. 
%First of all, we model edge weights as categories, 
%which works well for binned edge weights in practice but is theoretically dissatisfying. 
%Therefore, a natural enhancement of \ourmethod would be able to handle real edge weights, 
%possibly using a maximum entropy model on its edge weight distribution.
%Second, we currently test all our graph patterns at the same alpha level. 
%While this is theoretically defensible, given that we combine our statistical test with a model selection criterion, 
%dynamically adjusting our alpha level might be an option worth exploring.
%Finally, \ourmethod is currently limited to groups of node-aligned graphs, 
%and extending it to other graph types constitutes an interesting opportunity for future work.
%\begin{itemize}
%	\item background knowledge/prior
%	\item noise robustness
%\end{itemize}

==> text/table-data.tex <==
% !TeX spellcheck = en_US
% !TeX root = paper_appendix.tex
\begin{tabular}{p{0.13\linewidth}p{0.4125\linewidth}rr}
	\toprule
	\bfseries \mbox{Dataset}& \bfseries Description & $k$ & $[c_i]$\\
	\midrule
	\multicolumn{4}{c}{Functional Brain Networks (undirected, unweighted)}\\
	\multicolumn{4}{c}{$n = 116$; $m\in[1\,320,1\,348]$}\\
	\midrule
	fbn-a&\mbox{TD vs. ASD, age $[15,20]$}&$2$&$[116,121]$\\
	fbn-a1&\mbox{ASD, age $[15,20]$}&$1$&$[116]$\\
	fbn-c&TD vs. ASD, age $\leq 9$&$2$&$[49,52]$\\
	fbn-c1&ASD, age $\leq 9$&$1$&$[49]$\\
	fbn-ac&TD vs. ASD~$\times$~a vs. c&$4$&$[49,121]$\\
	fbn-e&\mbox{TD vs. ASD, eyes closed}&$2$&$[136,158]$\\
	fbn-e1&ASD, eyes closed&$1$&$[136]$\\
	fbn-m&TD vs. ASD, males only&$2$&$[418,420]$\\
	fbn-m1&ASD, males only&$1$&$[420]$\\
	\midrule
	\multicolumn{4}{c}{Air Transportation Networks (directed, weighted)}\\ 
	\multicolumn{4}{c}{$n = 300$; $m\in [335,3\,533]$}\\
	\midrule
	atn&all $(2005$--$2020)$&$1$&$[374]$\\
	atn-m&major carriers&$1$&$[191]$\\
	atn-n&national carriers&$1$&$[183]$\\
	atn-c&carrier classes&$2$&$[183,191]$\\
	%atn-s&season $[10,3]$ vs. $[4,9]$&$2$&$[185,189]$\\
	%atn-sc&season and carrier class&$4$&$[90,96]$\\
	%atn-q1&quarters from Jan&$4$&$[92,95]$\\
	atn-q&quarters $[12,3,6,9)$&$4$&$[92,95]$\\
	%atn-q3&quarters from Nov&$4$&$[93,94]$\\
	atn-y&four-year intervals&$4$&$[86,96]$\\
	\midrule
	\multicolumn{4}{c}{International Trade Networks (directed, weighted)}\\
	\multicolumn{4}{c}{$n = 250$; $m\in [256,11\,415]$}\\
	\midrule
	itn&all $(1989$--$2018)$&$1$&$[3\,976]$\\
	itn-p&product class&$5$&$[210,1\,530]$\\
	itn-y&ten-year intervals&$3$&$[1\,314,1\,332]$\\
	itn-py&product class~$\times$~intervals&$15$&$[70,510]$\\
	itn-a&animals&$1$&$[210]$\\
	itn-ay&animals in intervals&$3$&$[70,70]$\\
	itn-v&vegetables&$1$&$[796]$\\
	itn-vy&vegetables in intervals&$3$&$[247,262]$\\
	itn-f&food products&$1$&$[1\,137]$\\
	itn-fy&\mbox{food products in intervals}&$3$&$[377,380]$\\
	itn-m&minerals&$1$&$[330]$\\
	itn-my&mineral in intervals&$3$&$[110,110]$\\
	itn-c&chemicals&$1$&$[1\,530]$\\
	itn-cy&chemicals in intervals&$3$&$[510,510]$\\
	\bottomrule
\end{tabular}

==> text/table-notation.tex <==
% !TeX spellcheck = en_US
% !TeX root = ../paper_appendix.tex
\begin{tabular}{rl}\toprule
	\bfseries Symbol&\bfseries Definition \\\midrule
	$\cG$ & Set of graphs\\
%	\color{red} $j$ ($N$) $\rightarrow$ $|\cG|$& $|\cG|$\\
	$\Pi$ & Partition of $\cG$\\
	$k$& $|\Pi|$\\ % was l intermittently
	$\cG_i$ & Group of graphs, $\cG_i\subseteq \cG$, $\cG_i\in \Pi$\\
	$c_i$&$|\cG_i|$\\
	$G_i$ & $(V,E_i)$, graph $i$\\
	$V$ & Node set (the same across all graphs)\\
	$n$  & $|V|$\\
	$E_i$& Edge set of graph $i$\\
	$m_i$&$|E_i|$\\
	$W$&Edge categories or discrete edge weights\\
	$\cE$&$V \times V \times W$\\
	$2^{\cE}$&Power set of $\cE$\\
	$X$ &Set of edges, $X\subseteq \cE$\\
	$V_X$&Set of nodes incident with an edge in $X$\\
	$q_i(X)$&Empirical frequency of $X$ in $\cG_i$\\
	$S$&Set of edge sets, $S\subseteq 2^{\cE}$\\
	$p_i(X\mid S)$&Expected frequency of $X$ in $\cG_i$ under $S$\\
	$f$&Maximum entropy distribution\\
	$\theta_i$&Real-valued model parameter\\
	$A$&Association matrix\\
	$S_i$&$\{X\in S \mid A_{iX} = 1\}$\\
	$\ell(S)$&Log likelihood of $S$\\
	$\Delta(X)$&$\ell(S) - \ell(S \cup \{X\}) - |\Pi|/2\log |\cG| $\\
	$h(X)$&Heuristic approximation of $\Delta(X)$\\
	$\gamma$&Largest connected component size of $G\in \cG$\\
	\bottomrule
\end{tabular}

==> text/table-results.tex <==
% !TeX spellcheck = en_US
% !TeX root = paper.tex
\begin{tabular}{lrrrrrr}
	\toprule
	\bfseries
	Dataset&$c$&$\min$&$\max$&$\mu$&$\sigma$&$\chi$\\
	\midrule
	fbn-a&$99$ & $2$ & $29$ & $8$ & $5$ & $86$\\
	fbn-a1&$350$ & $2$ & $34$ & $7$ & $5$ & $-$\\
	fbn-c&$11$ & $3$ & $90$ & $20$ & $24$ & $1$\\
	fbn-c1&$29$ & $3$ & $99$ & $20$ & $19$ & $-$\\
	fbn-ac&$28$ & $2$ & $19$ & $4$ & $4$ & $2$\\
	fbn-e&$186$ & $2$ & $38$ & $7$ & $5$ & $166$\\
	fbn-e1&$531$ & $2$ & $35$ & $6$ & $4$ & $-$\\
	fbn-m&$1\,840$ & $2$ & $25$ & $3$ & $2$ & $1\,626$\\
	fbn-m1&$2\,508$ & $2$ & $22$ & $3$ & $2$ & $-$\\
	\midrule
	atn & $1\,709$ & $2$ & $148$ & $3$ & $6$ & $-$ \\
	atn-m & $2\,781$ & $2$ & $238$ & $3$ & $8$ & $-$ \\
	atn-n & $877$ & $2$ & $10$ & $2$ & $1$ & $-$ \\
	atn-c & $6$ & $14$ & $125$ & $46$ & $37$ & $1$ \\
	atn-q & $12$ & $5$ & $249$ & $92$ & $86$ & $5$ \\
	atn-y & $12$ & $6$ & $142$ & $53$ & $32$ & $10$ \\
	% OLD NUMBERS BELOW FOR COMP
%	atn&$1\,684$&$2$&$148$&$3$&$6$&$-$\\
%	atn-m&$2\,789$&$2$&$238$&$3$&$7$&$-$\\
%	atn-n&$873$&$2$&$10$&$2$&$1$&$-$\\
%	atn-c&$7$&$2$&$125$&$41$&$39$&$1$\\
%	atn-q&$15$&$2$&$287$&$73$&$98$&$6$\\
%	atn-y&$10$&$37$&$142$&$62$&$30$&$10$\\
	\midrule
	itn&$628$ & $2$ & $120$ & $4$ & $9$ & $-$\\
	itn-p&$10$ & $2$ & $28$ & $5$ & $8$ & $10$\\
	itn-y&$13$ & $9$ & $134$ & $44$ & $35$ & $10$\\
	itn-py&$14$ & $2$ & $72$ & $11$ & $19$ & $14$\\
	itn-a&$1012$ & $2$ & $123$ & $3$ & $7$ & $-$\\
	itn-ay&$10$ & $45$ & $92$ & $67$ & $16$ & $10$\\
	itn-v&$447$ & $2$ & $84$ & $4$ & $7$ & $-$\\
	itn-vy&$10$ & $12$ & $73$ & $36$ & $16$ & $10$\\
	itn-f&$878$ & $2$ & $87$ & $3$ & $6$ & $-$\\
	itn-fy&$24$ & $3$ & $73$ & $26$ & $22$ & $23$\\
	itn-m&$1\,260$ & $2$ & $119$ & $3$ & $7$ & $-$\\
	itn-my&$13$ & $6$ & $170$ & $73$ & $44$ & $11$\\
	itn-c&$1\,150$ & $2$ & $134$ & $3$ & $8$ & $-$\\
	itn-cy&$12$ & $7$ & $112$ & $60$ & $28$ & $10$\\
	% OLD NUMBERS BELOW FOR COMP
%	itn&$627$ & $2$ & $120$ & $4$ & $9$ & $-$\\
%	itn-p&$10$ & $2$ & $28$ & $5$ & $8$ & $11$\\
%	itn-y&$13$ & $9$ & $132$ & $44$ & $34$ & $10$\\
%	itn-py&$15$ & $2$ & $72$ & $12$ & $18$ & $$\\
%	itn-a&$1\,007$ & $2$ & $123$ & $3$ & $7$ & $-$\\
%	itn-ay&$11$ & $48$ & $92$ & $65$ & $15$ & \\
%	itn-v&$467$ & $2$ & $84$ & $3$ & $6$ & $-$\\
%	itn-vy&$11$ & $12$ & $74$ & $41$ & $17$ & \\
%	itn-f&$869$ & $2$ & $109$ & $3$ & $6$ & $-$\\
%	itn-fy&$22$ & $5$ & $88$ & $30$ & $22$ & \\
%	itn-m&$1\,250$ & $2$ & $119$ & $3$ & $7$ & $-$\\
%	itn-my&$12$ & $8$ & $108$ & $53$ & $31$ & \\
%	itn-c&$1\,188$ & $2$ & $128$ & $3$ & $7$ & $-$\\
%	itn-cy&$12$ & $10$ & $103$ & $65$ & $23$ & \\
	\bottomrule
\end{tabular}

==> text/table-synthetic.tex <==
% !TeX spellcheck = en_US
% !TeX root = paper_appendix.tex
	\begin{tabular}{rrcccc}
	\toprule
	\bfseries $k$& $p$ &\bfseries $P(|P|)$ & \bfseries Prevalence & \bfseries Position & $t$\\
	\midrule
	\multirow{2}{*}{$1$}&$0.2$&\multirow{2}{*}{\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		\text{cl}(5)\\\text{st}(1,9)\\\text{bc}(5,5)
	\end{bmatrix}$}&\setlength\arraycolsep{1.5pt}\tiny$\begin{bmatrix}
0.2&0.2&0.2
\end{bmatrix}^T$&\multirow{2}{*}{\setlength\arraycolsep{1.5pt}\tiny$\begin{bmatrix}
	0\\5\\15
\end{bmatrix}$}&\multirow{2}{*}{--}\\
	&$0.1$&&\setlength\arraycolsep{1.5pt}\tiny$\begin{bmatrix}
		0.1&0.2&0.3
	\end{bmatrix}^T$&&\\
	\midrule
	\multirow{3}{*}{$2$}&\multirow{3}{*}{$0.2$}&\multirow{3}{*}{$\text{st}(1,9)$}&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.2&0.2
	\end{bmatrix}$&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
	0&0
\end{bmatrix}$&s\\
	&&&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.2&0.4
	\end{bmatrix}$&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
	0&0
\end{bmatrix}$&c\\
	&&&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.4&0.4
	\end{bmatrix}$&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
	0&10
\end{bmatrix}$&c\\
	\midrule
	\multirow{3}{*}{$2$}&\multirow{3}{*}{$0.2$}&\multirow{3}{*}{$\text{cl}(5)$}&\multirow{3}{*}{\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.2&0.2
	\end{bmatrix}$}&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
0&0
\end{bmatrix}$&s\\
 	&&&&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
 		0&2
 	\end{bmatrix}$&o\\
	&&&&\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0&5
	\end{bmatrix}$&c\\
	\midrule
	\multirow{5}{*}{$4$}&$0.2$&\multirow{5}{*}{\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		\text{cl}(5)\\\text{cl}(5)\\\text{st}(1,9)\\\text{st}(1,9)\\\text{bc}(5,5)
	\end{bmatrix}$}&
	\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.2 & 0.2 & 0 & 0 & 0\\
		0 & 0.2 & 0.2 & 0 & 0\\
		0 & 0 & 0.2 & 0.2  & 0\\
		0 & 0 & 0 & 0.2 & 0.2\\
	\end{bmatrix}^T$&\multirow{5}{*}{\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
	0\\5\\10\\20\\30
\end{bmatrix}*4$}&\multirow{5}{*}{\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
\text{c}\\\text{s}\\\text{s}\\\text{s}\\\text{c}
\end{bmatrix}$}\\
&&&&&\\
	&$0.1$&&\tiny\setlength\arraycolsep{1.5pt}$\begin{bmatrix}
		0.1 & 0.2 & 0 & 0 & 0\\
		0 & 0.1 & 0.2 & 0 & 0\\
		0 & 0 & 0.3 & 0.2  & 0\\
		0 & 0 & 0 & 0.3 & 0.2\\
	\end{bmatrix}^T$&&\\
	\bottomrule
\end{tabular}
